Satellite Chasers: Divergent Adversarial Reinforcement Learning to Engage Intelligent Adversaries on Orbit

As space becomes increasingly crowded and contested, robust autonomous capabilities for multi-agent environments are gaining critical importance. Current autonomous systems in space primarily rely on optimization-based path planning or long-range orbital maneuvers, which have not yet proven effective in adversarial scenarios where one satellite is actively pursuing another. We introduce Divergent Adversarial Reinforcement Learning (DARL), a two-stage Multi-Agent Reinforcement Learning (MARL) approach designed to train autonomous evasion strategies for satellites engaged with multiple adversarial spacecraft. Our method enhances exploration during training by promoting diverse adversarial strategies, leading to more robust and adaptable evader models. We validate DARL through a cat-and-mouse satellite scenario, modeled as a partially observable multi-agent capture the flag game where two adversarial ``cat" spacecraft pursue a single ``mouse" evader. DARL's performance is compared against several benchmarks, including an optimization-based satellite path planner, demonstrating its ability to produce highly robust models for adversarial multi-agent space environments.

==> results.tex <==

\subsection{Experimental Setup}

In simulation, the dynamics of the evader and adversary spacecrafts can be described using the Clohessy Wiltshire (CW) Equations, which model the behavior of a spacecraft in relation to a single point moving on a near circular orbit:
\vspace{-2mm}
\begin{align}
\ddot{x} = 3n^2x + 2n\dot{y} + \frac{T_x}{m}
\label{eq:cwx}
\end{align}
\vspace{-4mm}
\begin{align}
\ddot{y} = -2n\dot{x} + \frac{T_y}{m}
\label{eq:cwy}
\end{align}
\vspace{-4mm}
\begin{align}
\ddot{z} = -n^2z + \frac{T_z}{m}
\label{eq:cwz}
\end{align}

Where $x,y,$ and $z$ are the Cartesian coordinates of the spacecraft relative to the single moving point, which is treated as the origin of out localized coordinate frame.

The cat and mouse training prompt is described in previous sections. During testing, both adversary and evader spacecrafts are given the same physical parameters (mass, inertia, etc.). Adversaries are modeled as a ball with a $1m$ radius, and represented as a point cloud. The evader must successfully come within $3m$ of a goal point, and return to its starting position without coming within $1m$ of an adversary for the episode to be considered successful. If the evader is capable of reaching the first goal but not returning to its starting position the episode is considered a partial success. And, if the evader does not reach either goal the episode is considered a failure.

In order to provide an impartial and standardized comparison of model performance, all models are tested in an environment with hand designed heuristic adversarial policies which receive expert knowledge of the nature of the cat and mouse game. Two expert adversarial policies are implemented, one that attempts to collide with the evader, and a second that attempts to block any path from the evader to the goal point. In every test episode, one of each heuristic policy is designated to a single adversary. The heuristic policy implemented is shown in Algorithm \ref{algo:adv}, where $h()$ is a function that determines the point the adversary should travel to, and $c()$ computes the desired action input.

\begin{algorithm}[t]
\caption{Adversary Heuristic Policy}
\label{algo:adv}
\begin{algorithmic}[1]
\State Initialize adversary at $\boldsymbol{p}_a$
\For{every timestep}
\State collect observation $\boldsymbol{s}_a$
\For{every $N$ steps}
\State $\boldsymbol{g}_a \leftarrow h(\boldsymbol{s}_a)$
\EndFor
\State $\boldsymbol{a}_a \leftarrow c(\boldsymbol{g}_a,\boldsymbol{s}_a)$
\State take action $\boldsymbol{a}_a$
\EndFor
\end{algorithmic}
\end{algorithm}


\subsection{Evaluation Benchmarks}
\label{subsec:eval}



Several methods are used as benchmarks in order to demonstrate our methods robustness, and ability to successfully evade intelligent adversaries, the several benchmarks are listed below. 

\begin{enumerate}
    \item \textit{EVADE}: EVADE is a optimization based path planner designed specifically for spacecraft operating in non-cooperative space environments with passive obstruction \cite{Mehlman2024-az}.

    \item \textit{Base Evader Policy (BE)}: This is the resulting policy of Stage I of training before it is retrained in Stage II.

    \item \textit{Single Adversary (SA)}: This method entails a single adversarial policy, thus no $\mathcal{L}_{KL_i}$ term and a standard linear activation.

    \item \textit{Base Multi-Adversary (MA)}: This method entails multiple adversarial policies, however, uses a standard linear activation and no $\mathcal{L}_{KL_i}$ term.

    \item \textit{DARL}: This is our full method discussed in Section \ref{sec:method}. The model is trained with 2 divergent adversarial policies.

    \item \textit{No Sine Activation (NSA)}: As a brief ablation demonstration, this implementation of our method uses a standard linear activation layer for the actor network.
\end{enumerate}


Methods 3-6 are all trained using the two stage training scheme discussed in Section \ref{sec:method}. Methods which include multiple adversaries entail training 2 separate policies. 


\subsection{Results and Discussion}

\begin{figure}[thpb]
      \centering
      {\includegraphics[scale=0.7]{img/combined_training_curve2.png}}
      \caption{Base evader training curve (left), and DARL, MA, and BA Evader training curves (right). The dotted red line marks the beginning of the evader policy's network updates.}
\label{fig:be_curve}
\end{figure}


\begin{table}
    \centering
    \caption{Average performance of models trained using benchmark methods listed in Section \ref{subsec:eval}.}
    \ra{1.1}
    \begin{tabular}{ccc}
        \midrule
         Method & Failure (\%) & Success (\%)\\
         \midrule
         EVADE & $100\%$ &  $0\%$ \\
         BE &  $58.7\%$ & $7.32\%$ \\
         SA & $40\%$  & $26\%$\\
         MA & $35.5\%$  & $36.5\%$\\
         \textbf{DARL} & $\mathbf{29\%}$  & $\mathbf{48.5}\%$\\
         NSA & $32\%$  & $40\%$\\
         \midrule
    \end{tabular}
    \label{tab:res}
\end{table}

Training curves for the baseline, DARL, MA, and SA evader can be seen in Figure \ref{fig:be_curve}. In the figure, the Evader Update Start line is placed at 12M timesteps, which was chosen in order to provide the adversarial policies with sufficient training to converge on a policy. Table \ref{tab:res} shows the test performance of each method where a failure or success is defined by the requirements stated earlier. In Table \ref{tab:res} it can be clearly seen that DARL outperforms all benchmarks both in maximizing successful episodes, and minimizing failures. It should also be noted that our two staged method clearly demonstrates the ability to produce policies for satellite autonomy that can perform in highly contested environments that standard satellite path-planning algorithms (EVADE) fail in. Although EVADE and the base evader are intended for partially-observable non-cooperative environments, neither were designed to protect a spacecraft in a strategic multi-agent game. Additionally, Table \ref{tab:res} shows that the top 3 performing models all involve training on multiple adversarial models, emphasizing the value gained from training in environments that force the learning policy to widen their exploration of the state space. 

In addition to comparing the testing performance of the models trained, Figure \ref{fig:val_curve} shows the average test performance of several methods throughout training. The Figure compares the average test performance of the policies trained through the Single-Adversary (SA), Multi-Adversary (MA), and DARL methods starting once the evader model begins updates. It should be noted that a base evader trained on multiple divergent adversaries both learns faster, and consistently learns more robust behavior for cat and mouse games.


\begin{figure}[thpb]
      \centering
      {\includegraphics[scale=0.6]{img/validation_curve.png}}
      \caption{Validation curve comparing the average test performance of the DARL, MA, and SA models trained at different timesteps.}
\label{fig:val_curve}
\end{figure}

\subsection{Sim-to-real Feasibility and Applications}

Although we do not attempt sim-to-real transfer, we believe with a series of adjustments to our simulation environment the resulting DARL models can be integrated into our UAV testbed via the MAGPIE System which is designed to emulate spacecraft architecture and behavior \cite{Mehlman2025-yx}. Primarily, this would entail modifying the environment to emulate UAV that take positional commands rather than spacecraft. Although training a model to provide positional commands rather than force control would simplify the problem at hand, it would allow for integration of additional safety features often employed in UAV sim-to-real transfer \cite{Ugurlu2022-jm}. Additionally, as shown by previous works with sufficient domain randomization successful sim-to-real on UAVs is feasible \cite{Loquercio2020-dz}.

Outside of hardware test-beds, RL policies have yet to be implemented on spacecraft in operational environments. However, space provides an appealing setting for autonomous applications due to communications-denied environments, and risks inherent to human-in-the-loop spaceflight operations \cite{Tipaldi2022-ey}. Furthermore, modern satellites posses computing power capable of running standard RL models, which are generally smaller than models trained using other ML methods. Reduced launch cost and the associated increase in launch frequency of small satellites provides potential for running DARL on a satellite in coming year, an effort our team is actively seeking with potential sponsors. Future work concerning sim-to-real should also include developing safety measures and assurances around the cat-and-mouse interaction.
